Modeling the Data-Generating Process is Necessary for Out-of-Distribution Generalization

Recent empirical studies on domain generalization (DG) have shown that DG algorithms that perform well on some distribution shifts fail on others, and no state-of-the-art DG algorithm performs consistently well on all shifts. Moreover, real-world data often has multiple distribution shifts over different attributes; hence we introduce multi-attribute distribution shift datasets and find that the accuracy of existing DG algorithms falls even further. To explain these results, we provide a formal characterization of generalization under multi-attribute shifts using a canonical causal graph. Based on the relationship between spurious attributes and the classification label, we obtain realizations of the canonical causal graph that characterize common distribution shifts and show that each shift entails different independence constraints over observed variables. As a result, we prove that any algorithm based on a single, fixed constraint cannot work well across all shifts, providing theoretical evidence for mixed empirical results on DG algorithms. Based on this insight, we develop Causally Adaptive Constraint Minimization (CACM), an algorithm that uses knowledge about the data-generating process to adaptively identify and apply the correct independence constraints for regularization. Results on fully synthetic, MNIST, small NORB, and Waterbirds datasets, covering binary and multi-valued attributes and labels, show that adaptive dataset-dependent constraints lead to the highest accuracy on unseen domains whereas incorrect constraints fail to do so. Our results demonstrate the importance of modeling the causal relationships inherent in the data-generating process.

==> files/classifier.tex <==


\section{What do we want from our classifier}
DG goal is to do well on an unseen distribution. 

There can be many kinds of unseen distributions.
\begin{itemize}
    \item Causal 
    \begin{itemize}
        \item $Y|X$ changes between domains
        \item $P(Y)$ changes between domains 
        \item $P(X)$ changes between domains (does not matter provably)
        \item If only $P(Y)$ is changing, best bet is to learn $\beta$ such that $(y - \beta(x))$ remains invariant across domains. If $Y|X$ is also changing, then need to learn $\phi$ such that $\phi(x) \perp\!\!\perp E|Y$ (in addition to generative loss/ reconstruction of $X$ loss, and a loss for predicting $E$ for some small part of the representation). And then learn $\beta$ such that $(y - \beta(\phi(x)))$ remains invariant across domains. 
        \item The first step builds the representation that is not caused by environment (addresses $P(Y|X)$ changing across domains). The second step is to fit the common predictor. It can also be done as two heads of a VAE.
    \end{itemize}
    \item Anti-causal
    \begin{itemize}
        \item $P(X|Y)$ changes between domains
        \item $P(Y)$ changes between domains
        \item Two problems: $P(Y|X)$ is not a stable mechanism. And $P(Y)$ can change between domains.
        \item Solution: First, learn $\phi$ such that $\phi(x) \perp\!\!\perp E|Y$(in addition to reconstruction loss for X). Then learn an invariant $\beta$ s.t.  $(y- \beta(\phi(x)))$ remains invariant across domains, in adddition to ERM loss.
        \item The first step above avoids learning the trivial solution for $\phi$ that learns the environments. (e.g., different $\phi_i$ for different env). The second step tackles that $P(Y)$ is also changing.
    \end{itemize}
\end{itemize}

Why is it better? If we only do the second step, model can learn the environment (like IRM). If we only do the first step, the error of the model on different domains may not be the same. 

Another benefit is that the method remains same irrespective of causal or anti-causal.

If the above is true, then in Rotated MNIST, with this method, it should not matter which angle is test angle (assuming that it is a causal task). we should get equal accuracy for all angles.

\jk{\textbf{Questions:}
\begin{enumerate}
    \item Do we explicitly define domains and assume access to environments? Currently, we do not use domain information for regularization (conditioning on E not adding anything to the constraint)
    \begin{enumerate}
        \item What if we assume access to a concepts vector -- environment can be one attribute of this vector. The questions are, \textbf{do we need a domain attribute} and \textbf{is it important to know which attribute is the domain}?\\
        E.g., Colored MNIST defined two domains with varying level of correlation b/w spurious feature and label, while CelebA assumes access to attribute values (gender, hair color) and a method like GroupDRO creates 4 domains using this, optimizing for the minority. Domains for all DG datasets in WILDS are created using metadata labels (attributes) provided -- there was no environment label beforehand. Considering these diverse settings, what should \textit{we} adopt? Can Colored MNIST work if domain was one of the attribute labels?\\\\
        \textbf{Another idea:} Can the graph communicate more about the attribute and constraints?\\
        E.g., domain variable + feature node in causal graph vs two interchangeable features/attributes\\
        \item Can environments be used in regularization? (proposing something which unites literature dealing with different terms can be useful).
    \end{enumerate}
    \item Additionally, do we need to justify access to this information? Maggie’s paper and paper on stress tests by Victor didn’t; but I guess since we are comparing to existing DG algos which do not access this metadata (except maybe Group DRO), it seems important.
\end{enumerate}
}

==> files/multi-attr_DG.tex <==
\section{Multi-attribute distribution shifts: DG algorithms fail to generalize}
\label{sec: multi-attr_distr_shift}


We focus on  representation learning-based~\citep{wang2021generalizing} DG algorithms, typically  characterized by a regularization term that constrains the standard ERM loss such as cross-entropy (see Table~\ref{table:baselines_constraints}). \textit{Which regularization constraint is the correct one?} This question has attracted much discussion~\citep{pmlr-v139-mahajan21b,ye2022ood,wiles2022a,johansson2019supportdomaininvariant,zhao2019learninginvariant} without resolution. Class-conditional independence of learnt representation and domain is a popular constraint but it was recently shown~\citep{pmlr-v139-mahajan21b} to be inadequate when the distribution of causal or stable features changes across domains. Many papers~\citep{johansson2019supportdomaininvariant,zhao2019learninginvariant,akuzawa2019adversarial} show that unconditional independence between the representation and domain is an incorrect constraint, yet it performs better than recent methods such as Invariant Risk Minimization~\citep{https://doi.org/10.48550/arxiv.1907.02893} on benchmark datasets  when the spurious attribute is varied independently of the class label~\citep{ye2022ood,pmlr-v139-mahajan21b}. Moreover, recent empirical work~\citep{ye2022ood,wiles2022a} shows that different algorithms perform better under different shifts, but none performs across all shifts. As a result, \citep{wiles2022a} suggests that instead of aiming for a universal algorithm for any shift, adaptable algorithms that use auxiliary attribute information can be more useful. 
%These results indicate that there might not be a single correct constraint\todo{cite Wiles et al.: "We should focus on the cases where we have knowledge about the distribution shift. Instead of trying to make one algorithm for any possible shift, it makes sense to have adaptable algorithms which can use auxiliary information if given.}.
% see pacs result in mahajan, diversity shift in ye

%\todo{possible caveat: we use the same constraint for the independent attribute case}
%\jk{simple case: distribution of Y, P(Y) changing across domains.} 

\begin{table}[h!]
  \caption{Statistic matched/optimized by different DG algorithms. $l$ represents the main classifier (class predictor) loss while $l_d$ is domain classifier loss. $h$ is a learnable domain classifier on top of shared representation $\phi$.}
  \label{table:baselines_constraints}
  \centering
  \begin{tabular}{ccc}
    \toprule
    \textbf{Constraint} & \textbf{Statistic} & \textbf{DG Algorithm} \\
    \midrule
    $\phi \perp\!\!\perp E$ & $\mathrm{match}\:\:\mathbb{E}[\phi(x)| E]\:\:\forall\:\:E$ & MMD~\citep{JMLR:v13:gretton12a} \\
    & $\max\:\:\ell_{d}(E, h(\phi(x)))$ & DANN~\citep{JMLR:v17:15-239} \\
    &  $\mathrm{match}\:\:\mathrm{Cov}[\phi(x)| E]\:\:\forall\:\:E$ & CORAL~\citep{10.1007/978-3-319-49409-8_35} \\
    \midrule
    $Y \perp\!\!\perp E|\phi$ & $\mathrm{match}\:\:\mathbb{E}[Y|\phi(x), E]\:\:\forall\:\:E$ & IRM~\citep{https://doi.org/10.48550/arxiv.1907.02893}\\
    & $\mathrm{match}\:\:\mathrm{Var}[l|E]\:\:\forall\:\:E$ & VREx~\citep{pmlr-v139-krueger21a}\\
    \midrule
    $\phi \perp\!\!\perp E|Y$ & $\mathrm{match}\:\:\mathbb{E}[\phi(x)| E, Y=y]\:\:\forall\:\:E$ & C-MMD~\citep{8578664}\\
    & $\max\:\:\ell_{d}(E, h(\phi(x))|Y=y)$ & CDANN~\citep{li2018adversarialcada} \\
    \bottomrule
  \end{tabular}
\end{table}

To explore this question further, while the above efforts consider domains with a single distribution shift, we consider a more realistic setup where each domain can have multiple shifts over different attributes (Figure~\ref{fig:main_fig_mnist}). We construct a multi-attribute dataset by combining two popular DG datasets: Rotated MNIST~\citep{7410650} where each domain has a different rotation angle and Colored MNIST~\citep{https://doi.org/10.48550/arxiv.1907.02893} where each domain has a different correlation of color with the label. Each domain $E_i$ has a specific rotation angle $r_i$ and a specific correlation $corr_i$ between color $C$ and label $Y$. Our setup consists of 3 domains: $E_1, E_2 \in \mathcal{E}_{tr}$ (training), $E_3 \in \mathcal{E}_{te}$ (test). We define $corr_i = P(Y=1|C=1) = P(Y=0|C=0)$ in $E_i$. In our setup, $r_1 = 15^{\circ}, r_2 = 60^{\circ}, r_3 = 90^{\circ}$ and $corr_1 = 0.9, corr_2 = 0.8, corr_3 = 0.1$ (see Suppl.~\ref{app:datasets} for details). All environments have 25\% label noise consistent with ~\citep{https://doi.org/10.48550/arxiv.1907.02893}. For multiple DG algorithms, we compare their test domain accuracy on \textit{color}, \textit{rotation} and \textit{col+rot} shift datasets (Figure~\ref{fig:main_fig_mnist}c). Between \textit{color} and \textit{rotation}, the former is a comparatively harder task and all methods achieve worse than random accuracy, except IRM which obtains 50\%. However, once we combine the two shifts, IRM's accuracy drops to 39.6\% with a substantially high variance. %but the accuracy of DG algorithms drops significantly for the  \textit{color-only} shift. 
Overall, comparing to \textit{color-only} shift, there is $\sim$5-11\% drop in accuracy; while for some algorithms, the accuracy remains stable but the estimate has increased variance.

\jk{Now that we added \textit{CACM} to the table, it also shows a drop in accuracy; should we reframe a bit?}

% \begin{table}[h!]
%   \caption{Acc drop in multi-shift settings. Test-domain validation without early stopping (consistent with DomainBed). Obs: Drop in accuracy/high variance.}
%   \label{table:crmnist_acc_drop}
%   \centering
%   \begin{tabular}{lccc}
%     \toprule
%     \textbf{Algorithm} & \textbf{color-only} & \textbf{rotation-only} & \textbf{color+rotation}\\
%     \midrule
%     ERM & 30.9 $\pm$ 1.6 & 61.9 $\pm$ 0.5 & 25.2 $\pm$ 1.3\\
%     IRM & 50.0 $\pm$ 0.1 & 61.2 $\pm$ 0.3 & 39.6 $\pm$ 6.7\\
%     VREx & 30.3 $\pm$ 1.6 & 62.1 $\pm$ 0.4 & 23.3 $\pm$ 0.4\\
%     MMD & 29.7 $\pm$ 1.8 & 62.2 $\pm$ 0.5 & 24.1 $\pm$ 0.6\\
%     CORAL & 28.5 $\pm$ 0.8 & 62.5 $\pm$ 0.7 & 23.5 $\pm$ 1.1\\
%     DANN & 20.7 $\pm$ 0.8 & 61.9 $\pm$ 0.7 & 32.0 $\pm$ 7.8\\
%     C-MMD & 29.4 $\pm$ 0.2 & 62.3 $\pm$ 0.4 & 32.2 $\pm$ 7.0\\
%     CDANN & 30.3 $\pm$ 9.1 & 61.8 $\pm$ 0.2 & 30.8 $\pm$ 8.0\\
%     \bottomrule
%   \end{tabular}
% \end{table}



%That leaves us with IRM, $Y \perp\!\!\perp D| \phi$. IRM is a necessary, valid constraint according to the graph. However, it has three problems: 1) if there is no noise in the data, $\phi$ can learn Y perfectly and the constraint will be trivially true (find cite from Mahajan et al. paper figure); 2) if $\phi$ learns $D$, then also constraint is trivially satisfied (ruocheng chen et al.); 3) If the number of environments is not higher than the dimension of $X_a$, then IRM is not a sufficient condition (Rosenfeld et al., the risks of IRM). The first two are minor and can be fixed with appropriate initialization of IRM algorithm. But the third limitation is a fundamental flaw.
%So if we have datasets where the distribution of class-conditional causal features changes with environment (attributes), and the number of assumed associational features are equal or more than the number of domains, then there is no existing method that will work. The only correct existing method assumes that some  auxiliary attribute is known and uses a constraint on it (maggie's shortcut work, victor-alex stress tests work).



